TARo: Token-level Adaptive Routing for LLM Test-time Alignment

Large language models (LLMs) exhibit strong reasoning capabilities but typically require expensive post-training to reach high performance. Recent test-time alignment methods offer a lightweight alternative, but have been explored mainly for preference alignment rather than reasoning. To bridge this gap, we propose, Token-level Adaptive Routing (TARo), which steers frozen LLMs toward structured reasoning entirely at inference time. Specifically, we first train reward models on step-wise mathematical traces to capture fine-grained logical consistency signals, then introduce a learnable token-level router that automatically controls the guidance of the reward model to the base model. Extensive experiments show that TARo significantly improves reasoning performance by up to +22.4% over base model and +8.4% over existing token-level test-time alignment methods, while also boosting out-of-distribution clinical reasoning (MedXpertQA) and instruction following (AlpacaEval). Furthermore, TARo also generalizes from small to large backbones without retraining, extending test-time alignment from preference optimization to robust, cross-domain reasoning.

==> figures/alpha_highlight.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{images/colored_alpha_pred_taro_output_math500.png}
  \caption{Token-level visualization of the router weight $\hat{\alpha}_t$ (blue = low, red = high based on percentile) on TaRo output for question from MATH500 where higher $\hat{\alpha}_t$ indicates larger weight on reasoning reward model. Base Model = Qwen2.5-3B; Reasoning Reward Model = Qwen2.5-0.5B.\yunkai{Can you summarize why this aligns with our intuition of how reward model works? I only see the word "Given" in red as i expect}}
  \label{fig:alpha-highlight}
\end{figure}



==> figures/token_distribution.tex <==
\begin{figure}[h]
  \includegraphics[width=\linewidth]{example-image-golden}
  \caption{Predicted alpha distribution by dataset.}
  \label{fig:alpha-distribution}
\end{figure}


==> sections/dataset.tex <==
\label{sec:dataset}
See examples from dataset in Table \ref{tab:augmented-step-dpo}

==> sections/inference_appx_dump.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{TPS} & \textbf{GPU Mem. (\%)} & \textbf{QPS} \\
\midrule
\multirow{2}{*}{Qwen2.5-3B}  & GenARM              & 85.6 & 4.29  & 0.0651 \\
                              & TARo (Top-K logits) & 85.9 & 5.22  & 0.0448 \\
\midrule
\multirow{2}{*}{Llama3.1-8B} & GenARM              & 80.7 & 6.93  & 0.0141 \\
                              & TARo (Full logits)  & 32.5 & 10.45 & 0.0161 \\
\bottomrule
\end{tabular}
\caption{Throughput analysis on MATH500. TPS = tokens per second; QPS = queries per second. Note that these results reflect unoptimized implementations;  techniques such as speculative decoding and fully sharded data-parallel inference have not been applied. % could further close any gap.%} --> AR: I don't think it can close a gap but rather I just wanted to state this since the throughput might be considered low.
} 
\label{tab:throughput}
\end{table}

% \ar{
We additionally compare the inference-time efficiency of TARo against GenARM in Table~\ref{tab:throughput}, measured on a single node with 8$\times$H100 GPUs. TARo introduces a lightweight router module to dynamically adjust $\alpha$, and we find that throughput is comparable to GenARM when the Top-K logits design (Design ii) is used. Expanding to full logits (Design i) reduces throughput, particularly for large-vocabulary models such as Llama3.1-8B ($V=128{,}256$); however, vocabulary sizes appear to have stabilized in recent model releases (e.g., Qwen~2.5 at 151K vs.\ Qwen~3 at 151K), suggesting this overhead will not grow with newer models. We report both tokens-per-second (TPS) and queries-per-second (QPS). QPS captures prompt caching benefits, which are amortized over generation length, and favoring more concise generations. % making QPS a more complete measure of end-to-end throughput. 


==> sections/limitation.tex <==
While our proposed token-level adaptive routing method demonstrates strong improvements in reasoning performance and generalization across domains and model scales, several limitations remain. First, the effectiveness of our approach is contingent on the quality of the reward model; if the reward model is poorly calibrated or misaligned with the target reasoning task, the guidance provided may be suboptimal or even detrimental. Second, our experiments primarily focus on mathematical and clinical reasoning benchmarks as well as AlpacaEval, and the generalizability of our method to other domains or more open-ended tasks remains to be fully explored. Third, although our router is lightweight and does not require retraining of the base model, it does introduce additional inference-time computation, which may impact latency in real-world applications. Finally, our ablation studies indicate that the optimal router configuration can vary across model families, suggesting that some manual tuning or domain expertise may still be required to achieve the best results. We encourage future work to address these limitations and further investigate the robustness and applicability of token-level adaptive routing in broader settings.

==> tables/augmented-step-dpo.tex <==
\begin{table}
  \centering
  \begin{tabular}{cll}
    \hline
    \textbf{Augmented}           & \textbf{Chosen} &  \textbf{Rejected} \\
    \hline
           &            &                           \\
   \checkmark     &      &                           \\
    \hline
  \end{tabular}
  \caption{\label{tab:augmented-step-dpo}
    Example of modified preference data with reasoning cues. Highlighted are verification and backtracking
  }
\end{table}

==> tables/diverse_domains_table_no_aug.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{lcccc}
    \hline
    \textbf{Method} & \textbf{MATH500} & \textbf{MedXpertQA} & \textbf{AlpacaEval} & \textbf{Average} \\
    \hline
    \multicolumn{5}{l}{\textit{Llama-3.1-8B Instruct Base \quad + \quad DeepSeek Distill Llama-8B Reward}} \\
    \hline
    \rowcolor{lightgray} UniR (same base)    & 51.2 & -- & -- & -- \\
    Llama-3.1-8B Instruct (Base)  & 32.0 & 13.0 & 17.3 & -- \\
    DeepSeek Llama-8B (Reward)    & 62.8 & 10.8  & 2.8 & -- \\
    GenARM*   & 48.6  & 11.6 & 12.3 &  \\
    Ours                          & 53.8 & -- & 20.2 & -- \\
    \hline
        \multicolumn{5}{l}{\textit{Qwen-2.5-3B Base \quad + \quad Qwen-2.5-0.5B Reward}} \\
    \hline
    \rowcolor{lightgray} UniR (same base and reward)     & 64.8 & -- & -- & -- \\
    Qwen-2.5 3B (Base)         &  & -- &  & -- \\
    Qwen-2.5 0.5B (Reward)         &  & -- &  & -- \\
    GenARM*   &  & -- &  & -- \\
    Ours                     & 60.4 & -- & 15.0 & -- \\
    \hline
    % \multicolumn{5}{l}{\textit{Qwen-3-4B Base \quad + \quad Qwen-3-4B Reward}} \\
    % \hline
    % Qwen-3 4B (Base)         & -- & -- & -- & -- \\
    % Qwen-4B (Reward)         & -- & -- & -- & -- \\
    % GenARM*   & -- & -- & -- & -- \\
    % Ours                     & -- & -- & -- & -- \\
    % \hline
    
  \end{tabular}
  \caption{\label{tab:diverse-methods}
    Performance across reasoning (MATH500, MedXpertQA) and instruction-following (AlpacaEval) benchmarks. Reward models are trained on data introduced in Section \ref{sec:dataset}. Prior test-time alignment methods (UniR) are shown in gray for comparison. * indicates we retrained with our data. Note UniR does not report on Qwen-3.
  }
\end{table*}

